LayoutFormer++: Conditional Graphic Layout Generation via Constraint Serialization and Decoding Space Restriction

Conditional graphic layout generation, which generates realistic layouts according to user constraints, is a challenging task that has not been well-studied yet. First, there is limited discussion about how to handle diverse user constraints flexibly and uniformly. Second, to make the layouts conform to user constraints, existing work often sacrifices generation quality significantly. In this work, we propose LayoutFormer++ to tackle the above problems. First, to flexibly handle diverse constraints, we propose a constraint serialization scheme, which represents different user constraints as sequences of tokens with a predefined format. Then, we formulate conditional layout generation as a sequence-to-sequence transformation, and leverage encoder-decoder framework with Transformer as the basic architecture. Furthermore, to make the layout better meet user requirements without harming quality, we propose a decoding space restriction strategy. Specifically, we prune the predicted distribution by ignoring the options that definitely violate user constraints and likely result in low-quality layouts, and make the model samples from the restricted distribution. Experiments demonstrate that LayoutFormer++ outperforms existing approaches on all the tasks in terms of both better generation quality and less constraint violation.

==> sections/backup/_ablations.tex <==
\subsection{Ablation Studies}
\label{sec:ablation}

\input{./sections/tables/ablations}

In Table~\ref{Tab:constrained_quantitative_results} and Table~\ref{Tab:other_quantitative_results}, we consider the model using Transformer encoder-decoder architecture and the alphabetic order for both the input and output sequences.
We denote it as \emph{EncDec-A}.
As discussed in Section~\ref{sec:approach}, there are other model variants.
The first one uses position order for the output sequences, denoted as \emph{EncDec-P}.
The second one leverages Transformer decoder only architecture, denoted as \emph{Dec-A}.
Table~\ref{Tab:ablation} compares their performance on RICO.
We underline the results where EncDec-A outperforms Dec-A.
It is observed that EncDec-A has advantages over Dec-A on refinement, Gen-T, Gen-TS and Gen-R, and performs closely or a little worse than Dec-A on UGen and completion.
Compared to UGen and completion, refinement, Gen-T, Gen-TS and Gen-R have more complex user needs and thus more complicated input sequences.
This is consistent with our intuition that the bidirectional Transformer encoder is superior in modeling complex sequences.
Besides, we use italic to denote better results between EncDec-A and EncDec-P.
We find that while EncDec-P outperforms EncDec-A on more metrics, their performance is quite similar most of the time.

% \input{./sections/tables/violation}
% Moreover, we study the effectiveness of the constrained decoding strategy on Gen-R. 
% We count how many relationships specified in the input are violated and use it as the metric.
% Table~\ref{Tab:violation_relation} show the results, where \unilayout{} and  \unilayout{}-Naive denote the versions with and without constrained decoding strategy.
% It is shown that the violation rate is reduced significantly by leveraging the constrained decoding strategy. 
% Besides, we also compare \unilayout{} with baselines.
% The results show that \unilayout{} outperforms all the baselines on PubLayNet but has a worse violation rate than CLG-LO on RICO.
% To figure out the reason, we revisit the quantitative and qualitative performance of CLG-LO on RICO in Table~\ref{Tab:quantitative_results} and Figure~\ref{fig:qualitative_rico}.
% We find that CLG-LO does not make a good trade-off: the aesthetic quality of layouts generated by CLG-LO is significantly worse than that of \unilayout{}.  



==> sections/backup/_constrained_layout_generation.tex <==
\input{./sections/tables/constrained_generation}
\input{./sections/tables/other_generation}
\begin{figure*}
    \centering
      \includegraphics[width=1.0\linewidth]{./figures/constrained_qualitative.pdf}
    \caption{Qualitative comparisons with baselines of constrained layout generation.}
    \label{fig:constrained_qualitative}
  \end{figure*}
  
  \begin{figure}
    \centering
      \includegraphics[width=1.0\linewidth]{./figures/other_qualitative.pdf}
    \caption{Qualitative comparisons with baselines of other layout generation}
    \label{fig:other_qualitative}
  \end{figure}
  
\subsection{Constrained Layout Generation}
\label{sec:experiment_constrained_generation}

\textbf{Baselines.} 
For the constrained layout generation tasks Gen-T, Gen-TS and Gen-R, we compare LayoutFormer++ against 1) \emph{NDN-none}~\cite{NDN}, \emph{LayoutGAN++}~\cite{LayoutGAN++} and \emph{BLT}~\cite{BLT} on Gen-T, 2) \emph{BLT}~\cite{BLT} on Gen-TS, 3) \emph{NDN}~\cite{NDN} and \emph{CLG-LO}~\cite{LayoutGAN++} on Gen-R. Besides, we also compare two model variants of our LayoutFormer++ as baselines to show the effect of the layout constrained decoding. The first one contains the same model architecture with LayoutFormer++, but do not leverage layout constrained decoding, which is denoted as \emph{Ours w/o Con.Dec.}. The second one is denoted as \emph{Ours w/o back}, which disable the roll back mechanism of LayoutFormer++. 

\textbf{Results and Analysis.}
Table~\ref{Tab:constrained_quantitative_results} shows the quantitative comparison on constrained layout generation\footnote{As we fail to reproduce NDN by ourselves, we directly use the results from \cite{LayoutGAN++} in Table~\ref{Tab:constrained_quantitative_results}. It is evaluated on simple datasets that only consider layouts with less than $10$ elements.}, and Figure~\ref{fig:constrained_qualitative} shows the qualitative comparison.

We first compare LayoutFormer++ with existing approaches on Gen-T, Gen-TS and Gen-R.  
In Table~\ref{Tab:constrained_quantitative_results}, we highlight the results of LayoutFormer++ by bold when they achieve the best performance among all the existing approaches.
On both two datasets and three constrained layout generation tasks, LayoutFormer++ achieve significantly better performance than the existing approaches on most quality metrics. 
For constraint violation, since existing approaches directly reset the generated layouts on Gen-T and Gen-TS, the violation rate makes no sense. LayoutFormer++ also makes no constraint violation on these two tasks. On the Gen-R task, LayoutFormer++ outperforms all the existing approaches on the Vio.\%, except CLG-LO on RICO. However, CLG-LO does not make a good trade-off: the aesthetic quality of layouts generated by CLG-LO is significantly worse than that of LayoutFormer++.
Same results can be obtain from the qualitative comparison. For each group in Figure~\ref{fig:constrained_qualitative}, the first column shows constraints from the user, and the other columns show the generated layouts from baselines. It can be found that LayoutFormer++ generates layouts with better spacing, less misalignment and fewer unreasonable overlaps, while achieve better constraint satisfaction especially on Gen-R.
This demonstrates that LayoutFormer++ not only can flexibly handle different user constraints, but also generate layouts with both better quality and constraint satisfaction than the existing task-specific approaches.

Then we compare the variants of LayoutFormer++ and have the following observations from Table~\ref{Tab:constrained_quantitative_results}.
Comparing to Ours w/o Con.Dec, Ours w/o back significantly decrease the constraint violation rate on almost every task and dataset, which demonstrates the advantage of the layout constrained decoding for the constraint satisfaction. However, Ours w/o back sometimes performs slightly worse on the quality metrics than Ours w/o Con.Dec. It make sense since it is difficult to make the trade-off between generation quality and the constraint satisfaction.
Comparing LayoutFormer++ with Ours w/o back, it can be observed that LayoutFormer++ improve the generation quality, and further decrease the constraint violation rate on Gen-R, which demonstrates the advantage of the roll-back mechanism. We underline the results of LayoutFormer++ when they achieve better performance than Ours w/o back.



==> sections/backup/_other_layout_generation.tex <==
\subsection{Other Layout Generation Tasks}
\label{sec:experiment_other_generation}

\textbf{Baselines.} 
To further demonstrate the capability of model generation, we evaluate LayoutFormer++ on the other various generation tasks includes UGen, Refinement and Completion.
We try our best to reproduce all the existing approaches.
Even so, we regret to not include some approaches for the following reasons.
First, due to the missing implementation details and hyperparameter settings, we fail to reproduce some approaches~\cite{LayoutGAN,attributelayoutgan,READ,layoutmcl}.
Second, a few approaches consider data-specific attributes and are difficult to be applied to arbitrary datasets about graphic layouts~\cite{content-aware,CanvasVAE}.
Ultimately,We compare LayoutFormer++ against 1) \emph{VTN}~\cite{VTN}, \emph{Coarse2Fine}~\cite{coarse2fine} and \emph{LayoutTransformer}~\cite{LayoutTransformer} on UGen, 2) \emph{RUITE}~\cite{RUITE} on refinement and 3) \emph{LayoutTransformer}~\cite{LayoutTransformer} on completion.

\textbf{Results and Analysis.}
Table~\ref{Tab:other_quantitative_results} shows the quantitative comparison and Figure~\ref{fig:other_qualitative} shows the qualitative comparison on UGen, Refinement and Completion task. As shown in Table~\ref{Tab:other_quantitative_results}, we highlight the results of LayoutFormer++ by bold when it achieve the best performance among the existing approaches. It can be observed that LayoutFormer++ outperforms on most metrics. In Figure~\ref{fig:other_qualitative}, each group shows generated layouts from baselines and LayoutFormer++. For completion, layouts in the same group are generated by giving the same element as the input. For refinement, in each group, the first column shows a layout draft from users, and the other columns show refined layouts from baseline and LayoutFormer++. We can observe that on UGen and completion task, LayoutFormer++ performs better at details. And for refinement, LayoutFormer++ can better improve the layout draft while keeping the overall layout design.

==> sections/backup/ablations.tex <==
\begin{table*}
    \centering
    \caption{Ablation studies on RICO.}
    \renewcommand{\arraystretch}{1.2}
    \begin{small}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{lcccccccccccc}
                \specialrule{1.1pt}{0pt}{1pt}
                         & \multicolumn{4}{c}{UGen}   & \multicolumn{4}{c}{Completion} & \multicolumn{4}{c}{Refinement}                                                                                                                                                                                                                           \\ \cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13}
                Model    & mIoU $\uparrow$            & FID $\downarrow$               & Align. $\downarrow$            & Overlap $\downarrow$ & mIoU $\uparrow$   & FID $\downarrow$           & Align. $\downarrow$ & Overlap $\downarrow$ & mIoU $\uparrow$            & FID $\downarrow$  & Align. $\downarrow$        & Overlap $\downarrow$ \\ \hline
                Dec-A    & 0.737                      & 10.513                         & 0.069                          & 0.566                & 0.734             & 2.213                      & 0.117               & 0.542                & 0.814                      & 0.039             & 0.208                      & 0.476                \\
                EncDec-P & 0.739                      & \textit{17.534}                & \textit{0.046}                 & \textit{0.453}       & \textit{0.783}    & 8.449                      & \textit{0.053}      & \textit{0.403}       & 0.814                      & \textit{0.031}    & \textit{0.116}             & \textit{0.486}       \\
                EncDec-A & \underline{\textit{0.742}} & 19.688                         & \underline{0.047}              & \underline{0.547}    & 0.732             & \textit{4.574}             & \underline{0.077}   & \underline{0.487}    & \underline{\textit{0.816}} & \underline{0.032} & \underline{0.123}          & 0.489                \\

                \specialrule{1.1pt}{0pt}{1pt}

                         & \multicolumn{4}{c}{Gen-T}  & \multicolumn{4}{c}{Gen-TS}     & \multicolumn{4}{c}{Gen-R}                                                                                                                                                                                                                                \\ \cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13}
                Model    & mIoU $\uparrow$            & FID $\downarrow$               & Align. $\downarrow$            & Overlap $\downarrow$ & mIoU $\uparrow$   & FID $\downarrow$           & Align. $\downarrow$ & Overlap $\downarrow$ & mIoU $\uparrow$            & FID $\downarrow$  & Align. $\downarrow$        & Overlap $\downarrow$ \\ \hline
                Dec-A    & 0.410                      & 5.095                          & 0.323                          & 0.558                & 0.588             & 4.771                      & 0.161               & 0.617                & 0.428                      & 2.000             & 0.313                      & 0.539                \\
                EncDec-P & \textit{0.488}             & 2.679                          & \textit{0.060}                 & \textit{0.491}       & \textit{0.632}    & 1.861                      & \textit{0.136}      & \textit{0.491}       & \textit{0.496}             & \textit{1.290}    & 0.119                      & \textit{0.511}       \\
                EncDec-A & \underline{0.431}          & \underline{1.534}              & \underline{0.124}              & 0.702                & \underline{0.618} & \underline{\textit{0.775}} & \underline{0.151}   & \underline{0.547}    & 0.427                      & \underline{1.642} & \underline{\textit{0.097}} & 0.552                \\ % \cline{4-4}
                % EncDec-A & \underline{0.424}        & \underline{\textit{1.534}}     & \underline{0.124}              & \underline{0.540}    & \underline{0.618}}& \underline{\textit{0.775}} & \underline{0.151}   & \underline{0.547}    & 0.420                      & 6.293             & \underline{\textit{0.109}} & 0.547                \\
                \specialrule{1.1pt}{1pt}{0pt}
            \end{tabular}}
    \end{small}
    \label{Tab:ablation}
\end{table*}

==> sections/backup/comparison_of_constraint_serialization.tex <==
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
        \resizebox{0.95\linewidth}{!}{
            \begin{tabular}{llcccc}
                \specialrule{1.1pt}{0pt}{1pt}
                                            &                       & \multicolumn{4}{c}{RICO}    \\ 
                                            \cmidrule(l){3-6}  
                Tasks                       & \makecell{Order}      & mIoU $\uparrow$   & FID $\downarrow$  & Align. $\downarrow$   & Overlap $\downarrow$  \\ \hline
                \multirow{2}{*}{Gen-T}      & by element            & 0.360             & 46.483            & 0.128                 & 0.676                 \\ 
                                            & by constraint         & \textbf{0.742}    & \textbf{19.688}   & \textbf{0.047}        & 0.547     \\
                                            \hline
                \multirow{2}{*}{Gen-R}      & by element            & 0.811             & 0.107             & 0.133                 & 0.483                 \\ 
                                            & by constraint         & \textbf{0.816}    & \textbf{0.032}    & \textbf{0.123}        & 0.489 \\
                                            \hline
                \multirow{2}{*}{Refinement} & by element            & 0.363             & 6.679             & 0.194                 & 0.478                 \\
                                            & by constraint         & \textbf{0.732}    & \textbf{4.574}    & \textbf{0.077}        & 0.487         \\ 
                \specialrule{1pt}{1pt}{1pt}
                \specialrule{1pt}{1pt}{1pt}
                                            &                       & \multicolumn{4}{c}{PubLayNet}    \\ 
                                            \cmidrule(l){3-6}  
                Tasks                       & \makecell{Order}      & mIoU $\uparrow$   & FID $\downarrow$  & Align. $\downarrow$   & Overlap $\downarrow$  \\ \hline
                \multirow{2}{*}{Gen-T}      & by element            & 0.360             & 46.483            & 0.128                 & 0.676                 \\ 
                                            & by constraint         & \textbf{0.742}    & \textbf{19.688}   & \textbf{0.047}        & 0.547     \\
                                            \hline
                \multirow{2}{*}{Gen-R}      & by element            & 0.811             & 0.107             & 0.133                 & 0.483                 \\ 
                                            & by constraint         & \textbf{0.816}    & \textbf{0.032}    & \textbf{0.123}        & 0.489 \\
                                            \hline
                \multirow{2}{*}{Refinement} & by element            & 0.363             & 6.679             & 0.194                 & 0.478                 \\
                                            & by constraint         & \textbf{0.732}    & \textbf{4.574}    & \textbf{0.077}        & 0.487         \\ 
                \specialrule{1.1pt}{1pt}{0pt}
            \end{tabular}
        }
    \caption{Comparisons of different constraint serialization.}
    \label{tab:comparison_of_constraint_serialization}
\end{table}


==> sections/backup/old_intro.tex <==
% ========= old version =========

% Thus, besides generating high-quality layouts that accord with design principles (e.g., good alignment and proper space), it should also achieve \emph{good controllability}.
% two goals simultaneously and thus is much more challenging.
% Specifically, one goal is \emph{high quality}, meaning that generated layouts should accord with design principles (e.g., good alignment and proper space), and the other goal is \emph{good controllability}, standing for that generated layouts should conform to diverse user constraints (see Figure~\ref{}).

% To assist layout design, great interest has been aroused to the technologies about automatic layout generation.

% There are two requirements for the layout generation method: the \textit{quality} and the \textit{control}. In terms of the quality, it is required to generate real and complex layouts. Recent works~\cite{LayoutGAN++, VTN, CanvasVAE, coarse2fine, RUITE, LayoutTransformer, BLT} have made meaningful attempts in generating high-quality layouts by modeling layouts as sequences of element attributes. For the control, it requires from two aspects. First, the method is required to generate layout according to user intents. It should be emphasized that the method should be able to deal with multiple types of constraints given by the users rather than only certain one type, since the intents of each user are various in the practical scenario. Second, the method should take appropriate steps to ensure that the generated layouts conform user constraints, while maintain the quality and efficiency of the generation process. Although some of the mentioned works~\cite{LayoutGAN++, RUITE, LayoutTransformer, BLT} have considered some user constraints, unfortunately, none of them is able to achieve the control requirements.

% Existing work makes meaningful attempts on conditional layout generation.
% First, various user constraints are explored~\cite{}, e.g., refinement, completion, element types, element sizes and element relationships.
% Second, a layout is usually represented as a sequence of elements and their five attributes, including type, top coordinate, left coordinate, width and height.
% % by first concatenating five attributes of each element (including type, top coordinate, left coordinate, width and height) and then concatenating different elements~\cite{}.
% Third, Transformer~\cite{} is widely leveraged to achieve the state-of-the-art performance~\cite{}.

% most existing approaches simply use the same way to model user constraints and layouts.
% Specifically, they use the same sequence format to represent user constraints and layouts, and the same module to encode user constraints and generate layouts.
% (either a Transformer encoder or a Transformer decoder) 
% This makes existing methods limited in providing adequate controllability, i.e.,
% tackling diverse user constraints. For example, LayoutTransformer~\cite{} can only perform completion task and BLT~\cite{} cannot handle element relationships.
% Besides, this also makes existing methods fail to achieve satisfactory quality.
% Specifically, for user constraints, the global context is very important while for layouts, what has been generated is very important.
% Second, there are many limitations in ensuring the constraint compliance.

% To model the user constraint previous approaches~\cite{RUITE, LayoutTransformer, BLT} directly present the user constraints in the target layout sequence, which restricts the constraints to the element attributes. Besides, since the constraints and the target layout are represented in the same sequence, the model need to process constraints modeling and layout prediction simultaneously, which is hard to achieve good performance. 
% For the constraint exerting problem, previous work~\cite{RUITE, LayoutTransformer, BLT} directly reset the layout sequence by the given attributes to ensure the generated layout conforms the user given constraints. This damages the layout quality. Other works like~\cite{LayoutGAN++}, forcing the constraints by latent optimization after finishing the generation process, which is very complicated and time-consuming.

% In this work, we propose an approach named [Approach Name] for constrained layout generation, which is the first layout generation method that can completely achieve the control requirements. To solve the constraint modeling problem, we first design an identical format which could represent diverse constraints. Different from previous works give the attribute constraint in the same sequence of target layout, we construct separate constraint sequence from target layout. The intuition behind is two-fold. First, while users’ needs vary in different cases, they can all be formulated as independent sequences by tokens. Specifically, when the constraints are element attributes, these attributes can be concatenated to formulate a sequence. When handling other complex constraints, we can introduce new tokens to description them into the sequences, without any form limitations. 
% Second, since we separate the constraints sequence from target layout, we can use individual module for constraints modeling. In particular, we leverage an encoder-decoder based architecture for our model. The encoder processes the constraints in a bidirectional way, which could better model their context. The decoder predicts the layout sequence autoregressively, ensuring the generation quality by leveraging teacher-forcing during training.

% Second, to forcing the generated layout conforms the given constraints, it is naturally to exclude the values that will cause the violation of the constraints for the element attributes. Inspired by this, we introduce [Constrained Decoding Strategy] to our decoding process to solve the constraint exerting problem. As our decoder predicts the tokens of the layout sequence in an autoregressive way, [Constrained Decoding Strategy] considers both the already predicted attributes and the corresponding constraints to prune the infeasible values for the current token during each decoding step. 
% It is superior from two aspects to the previous works. First, different from the previous approaches directly reset tokens after the whole prediction, constrained decoding force the generation to conform the constraints while still taking advantage of the distribution learned from training data, which ensure the generation quality. Second, constrained decoding only needs to be leveraged in the inference decoding step, without requiring training for any additional module, which greatly improve the efficiency.

% [Approach Name] can flexibly tackle all the various user constraints through a single model, and significantly outperforms the previous task-specific approaches, achieves the requirements of both quality and control for layout generation.


% ========= old version =========

% There are two requirements for the layout generation method: the \textit{quality} and the \textit{control}. In terms of the quality, it is required to generate layouts as close to the real layouts as possible. Specifically, the generated layouts must have good diversity that contain both simple layouts and complex layout that with large number of elements. The placements of elements should conform to the aesthetic natures, such as aligning with each other and avoiding error overlap. In order to model the complicated relations between elements on the layout, Transformer~\cite{Transformer} has been introduced as the building blocks for layout generation model~\cite{LayoutGAN++, VTN, CanvasVAE, coarse2fine, RUITE, LayoutTransformer, BLT}. The most recent works~\cite{RUITE, LayoutTransformer, BLT} represent layout by a sequence of elements, where each element are represented by a sub-sequence of element attributes (see Figure~\ref{}). Drawing support from the attention mechanism, these approaches predict the attributes by learning the high-level relationships between each element, which make great progress in generating layout with high quality.

%  For the control, the layout generation method should be able to generate layout according to the user intent, which is the indispensable function in the practical application of layout generation. Various user constraints should be modeled, and be exerted over the generated layout. However, compared with the achievement gained in the quality, existing works still have many limitations in handling user constraints, which can be divided into three types. The first type of works~\cite{VTN, CanvasVAE, coarse2fine} does not model user constrained and only consider unconstrained layout generation task, which fails in the control. The second type of works~\cite{RUITE, LayoutTransformer, BLT} only considers element attributes as user constraints. They directly model these attribute constraints in the same format of target layout sequence, which can not be leveraged to other type of constraints. The way they ensure the conforms of the constraints is resetting the attributes in the generated layout by the given attributes. However, the direct reset will destroy the relationships between generated attributes, which inevitably lead to a decline in quality. The third type of works proposes special module to tackle certain constraints that beyond element attributes, such as latent optimization for element relationship constraints~\cite{LayoutGAN++}. Such module introduces additional computation that will reduce the generation efficiency, and is also hard to generalize to other constraints.

% In this paper, we propose a new approach to achieve both quality and control requirements for layout generation. To eliminate the control limitations, it is necessary to find a constraint format which can model all the different content. We find sequence is such format can easily represent all the different constraints and naturally processed by Transformer model without additional specially designed module. But different from previous works give the attribute constraint in the same sequence of target layout, we construct separate constraint sequence from target layout, so that constraints are not limited to the element attributes. Specifically, when the constraints are element attributes, these attributes will be concatenated into a sequence. When the constraints exceed the attributes, such as the relationships between elements, we introduce new tokens to description these constraints, and concatenate these tokens as constraint sequence.

% To exert the user constraints over generated layout, inspired by the constrained decoding from text generation, we propose layout constrained decoding strategy for our approach. During the autoregressive decoding process, constrained decoding strategy drops out the infeasible values that do not meet the given constraints for the current predicting token, i.e., the element attributes. It is superior from two aspects to the previous works. First, different from the previous approaches directly reset tokens after the whole prediction, constrained decoding force the generation to conform the constraints while still taking advantage of the distribution learned from training data, which ensure the generation quality. Second, constrained decoding only needs to be leveraged in the inference decoding step, without requiring training for any additional module, which greatly improve the efficiency.

% According to the way we format the user constraints, the layout generation task is modeled as a seq2seq generation task. We naturally leverage a Transformer encoder-decoder architecture for our model [Approach Name]. Comparing with the decoder-only and the encoder-only architecture used by previous works, the encoder-decoder architecture combine their advantages, where the bidirectional encoder can better capture the context of user constraints, and the autoregressive decoder ensures the generation quality of sequence. Therefore, our model can further improve the quality of generated layout.




==> sections/backup/old_related_work.tex <==
% Graphic layout generation is an emerging research topic. It aims at generating aesthetic layouts to tackle users' needs. 
% To achieve good performance on generating high-quality layouts, existing works have applied deep generative model to graphic layout generation. For example, GAN~\cite{LayoutGAN,content-aware,LayoutGAN++} and VAE~\cite{NDN,READ,VTN,coarse2fine,CanvasVAE} are the ones used most frequently. To better handle the high-level relationships between larger number of elements on one layout, Transformer with self-attention mechanism has been introduced as the important building blocks for the layout generation model~\cite{BLT,RUITE,LayoutGAN++,LayoutTransformer,VTN,coarse2fine,CanvasVAE}. Among these works, the most recent works LayoutTransformer~\cite{LayoutTransformer} and BLT~\cite{BLT} model the layout generation task as sequence generation and achieve the state-of-the art performance. LayoutTransformer~\cite{LayoutTransformer} represents the layout as a sequence of elements attributes and leverage a decoder-only Transformer model to predict the layout sequence autoregressively. BLT~\cite{BLT} use a Transformer encoder model to predict the masked attributes by attending to the unmasked attributes to complete the layout sequence. Based on the experience of these works, we also represent the layout as the sequence of element attributes, but leverage a Transformer encoder-decoder architecture to further improve the performance of the layout generation model.

% Besides the expectation of the quality, the layout generation method is also required to synthesize layouts that incorporate the user intents or constraints. Although some studies only focus on the unconstrained layout  generation~\cite{LayoutGAN,VTN,coarse2fine,CanvasVAE}, many of the previous works have explored different layout generation tasks with various user constraints. \cite{NDN,LayoutGAN++,BLT} study generating layouts from the user given element types. \cite{BLT} can also generate layouts condition on the element type and size. \cite{NDN,LayoutGAN++} synthesize layouts that conform the relative relationship among elements specified by user. \cite{RUITE} takes a rough layout as input and output a refined layout with better quality. \cite{LayoutTransformer} can complete the whole layout from the user given partial layout.
% However, previous methods are all designed specifically for certain constraints. Due to the constraint contents are quite different, none of existing works can cover all the layout generation tasks with different user constraints. In this work, we study the problem of modeling different user constraints, and propose a identical format for various constraints input which can be easily feed to the generation model.

% \textbf{Constrained Decoding.}
% Constrained decoding was first proposed for controllable text generation. Previous works~\cite{hokamp-liu-2017-lexically,anderson-etal-2017-guided} explore constrained beam search to exert lexical constraints, i.e. impose explicit phrase-based constraints to be placed on target output.
% \cite{post-vilar-2018-fast,hu-etal-2019-improved} further improve the efficiency of the constrained decoding method. 
% However, constrained layout generation not only suffers from multiple constraints, but also constrained by what have been placed on the canvas, which is much more complex than the lexical constraints in NLP. Thus, we adapt the constrained decoding into layout generation as [Layout Constrained Decoding], with fallback mechanism to solve the value problems caused by the conflict among the constraints.

==> sections/backup/other_generation.tex <==
% \begin{table*}
%     \centering
%     \caption{Quantitative comparisons with baselines.}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{small}
%         \resizebox{\textwidth}{!}{
%             \begin{tabular}{llcccccccc}
%                 \specialrule{1.1pt}{0pt}{1pt}
%                                             &                       & \multicolumn{4}{c}{RICO}   & \multicolumn{4}{c}{PubLayNet}    \\ 
%                                             \cmidrule(l){3-6}   \cmidrule(l){7-10}
%                 Tasks                       & \makecell{Methods}    & mIoU $\uparrow$   & FID $\downarrow$  & Align. $\downarrow$   & Overlap $\downarrow$  
%                                                                     & mIoU $\uparrow$   & FID $\downarrow$  & Align.  $\downarrow$  & Overlap  $\downarrow$       \\ \hline
%                 \multirow{4}{*}{UGen}       & LayoutTransformer     & 0.439             & 22.884            & 0.052                 & 0.471                      
%                                                                     & 0.062             & 36.304            & 0.031                 & 0.0009                      \\
%                                             & VTN                   & 0.686             & 76.064            & 0.461                 & 0.694                      
%                                                                     & 0.210             & 103.373           & 0.205                 & 0.211                       \\ 
%                                             & Coarse2Fine           & 0.360             & 46.483            & 0.128                 & 0.676                      
%                                                                     & 0.361             & 50.854            & 0.221                 & 0.142                       \\ 
%                                             & LayoutFormer++        & \underline{\textbf{0.742}}    & \underline{19.688}    & \underline{\textbf{0.047}}    & 0.547                      
%                                                                     & \underline{0.417}             & 46.522                & \underline{\textbf{0.029}}    & \underline{0.0009}    \\
%                                             \hline

%                 \multirow{2}{*}{Refinement} & RUITE                 & 0.811             & 0.107             & 0.133                 & 0.483                      
%                                                                     & 0.781             & 0.061             & 0.029                 & 0.020                       \\ % \cline{2-2}
%                                             & LayoutFormer++        & \underline{\textbf{0.816}} & \underline{\textbf{0.032}} & \underline{\textbf{0.123}} & \textbf{0.489}             
%                                                                     & \underline{\textbf{0.785}} & \textbf{0.086} & \underline{0.024} & \underline{\textbf{0.0055}} \\ % \cline{2-2}
%                                             \hline

%                 \multirow{2}{*}{Completion} & LayoutTransformer     & 0.363             & 6.679             & 0.194                 & 0.478                      
%                                                                     & 0.077             & 14.769            & 0.019                 & 0.0013                      \\ % \cline{2-2}
%                                             & LayoutFormer++S       & \underline{\textbf{0.732}} & \underline{4.574}  & \underline{0.077} & 0.487                      
%                                                                     & \underline{0.471}          & \underline{10.251} & \textbf{0.020}    & 0.0022                      \\ % \cline{2-2}
%                 \specialrule{1.1pt}{1pt}{0pt}
%             \end{tabular}}
%     \end{small}
%     \label{Tab:other_quantitative_results}
% \end{table*}


\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
        \resizebox{0.95\linewidth}{!}{
            \begin{tabular}{llcccc}
                \specialrule{1.1pt}{0pt}{1pt}
                                            &                       & \multicolumn{4}{c}{RICO}    \\ 
                                            \cmidrule(l){3-6}  
                Tasks                       & \makecell{Methods}    & mIoU $\uparrow$   & FID $\downarrow$  & Align. $\downarrow$   & Overlap $\downarrow$  \\ \hline
                \multirow{4}{*}{UGen}       & LayoutTransformer     & 0.439             & 22.884            & 0.052                 & 0.471                  \\
                                            & VTN                   & 0.686             & 76.064            & 0.461                 & 0.694                 \\ 
                                            & Coarse2Fine           & 0.360             & 46.483            & 0.128                 & 0.676                 \\ 
                                            & LayoutFormer++        & \textbf{0.742}    & \textbf{19.688}   & \textbf{0.047}        & 0.547     \\
                                            \hline
                \multirow{2}{*}{Refinement} & RUITE                 & 0.811             & 0.107             & 0.133                 & 0.483                 \\ 
                                            & LayoutFormer++        & \textbf{0.816}    & \textbf{0.032}    & \textbf{0.123}        & 0.489 \\
                                            \hline
                \multirow{2}{*}{Completion} & LayoutTransformer     & 0.363             & 6.679             & 0.194                 & 0.478                 \\
                                            & LayoutFormer++        & \textbf{0.732}    & \textbf{4.574}    & \textbf{0.077}        & 0.487         \\ 
                \specialrule{1pt}{1pt}{1pt}
                \specialrule{1pt}{1pt}{1pt}
                                            &                       & \multicolumn{4}{c}{PubLayNet}    \\ 
                                            \cmidrule(l){3-6}  
                Tasks                       & \makecell{Methods}    & mIoU $\uparrow$   & FID $\downarrow$  & Align. $\downarrow$   & Overlap $\downarrow$  \\ \hline
                \multirow{4}{*}{UGen}       & LayoutTransformer     & 0.062             & 36.304            & 0.031                 & 0.0009                  \\
                                            & VTN                   & 0.210             & 103.373           & 0.205                 & 0.211                 \\ 
                                            & Coarse2Fine           & 0.361             & 50.854            & 0.221                 & 0.142                 \\ 
                                            & LayoutFormer++        & \textbf{0.417}    & 46.522            & \textbf{0.029}        & \textbf{0.0009}     \\
                                            \hline
                \multirow{2}{*}{Refinement} & RUITE                 & 0.781             & 0.061             & 0.029                 & 0.020                 \\ 
                                            & LayoutFormer++        & \textbf{0.785}    & 0.086             & \textbf{0.024}        & \textbf{0.0055}        \\
                                            \hline
                \multirow{2}{*}{Completion} & LayoutTransformer     & 0.077             & 14.769            & 0.019                 & 0.0013                \\
                                            & LayoutFormer++        & \textbf{0.471}    & \textbf{10.251}   & 0.020                 & 0.0022         \\ 
                \specialrule{1.1pt}{1pt}{0pt}
            \end{tabular}
        }
    \caption{Quantitative comparisons with baselines of other layout generation tasks.}
    \label{Tab:other_quantitative_results}
\end{table}


